Systematic Use of Random Self-Reducibility against Physical Attacks

This work presents a novel, black-box software-based countermeasure against physical attacks including power side-channel and fault-injection attacks. The approach uses the concept of random self-reducibility and self-correctness to add randomness and redundancy in the execution for protection. Our approach is at the operation level, is not algorithm-specific, and thus, can be applied for protecting a wide range of algorithms. The countermeasure is empirically evaluated against attacks over operations like modular exponentiation, modular multiplication, polynomial multiplication, and number theoretic transforms. An end-to-end implementation of this countermeasure is demonstrated for RSA-CRT signature algorithm and Kyber Key Generation public key cryptosystems. The countermeasure reduced the power side-channel leakage by two orders of magnitude, to an acceptably secure level in TVLA analysis. For fault injection, the countermeasure reduces the number of faults to 95.4% in average.

==> tables/table_function_time.tex <==

\begin{table}[t]
  \small
  \centering
  \caption{Time of Functions.}
  \label{table_tdc_rms}
  \small
  \begin{tabular}{|p{3.5cm}|p{1.75cm}|p{1.75cm}|}
    \hline
    \textbf{Function}                     & \textbf{Clock Cycle } & \textbf{Time (us)}
    \\ \hline \hline
    Modulo Unprotected                    & 203
                                          & 1.21                                       \\ \hline
    Modulo Protected                      & 8840
                                          & 52.62                                      \\ \hline
    Modular Multiplication Unprotected    & 227
                                          & 1.35                                       \\ \hline
    Modular Multiplication Protected      & 12800                 & 76.19              \\ \hline
    Modular Exponentiation Unprotected    & 15704
                                          & 93.48                                      \\ \hline
    Modular Exponentiation Protected      & 325516                & 1937.60            \\ \hline
    Polynomial Multiplication Unprotected & 413
                                          & 2.46                                       \\ \hline
    Polynomial Multiplication Protected   & 21856                 & 130.10             \\ \hline
    NTT Unprotected                       & 8497
                                          & 50.58                                      \\ \hline
    NTT Protected                         & 195454                & 1163.42            \\ \hline
    Kyber Unprotected                     & 40890
                                          & 243.39                                     \\ \hline
    Kyber Protected                       & 890295                & 5299.38            \\ \hline
  \end{tabular}
\end{table}

